Online Human Activity Recognition using Low-Power Wearable Devices

Human activity recognition~(HAR) has attracted significant research interest due to its applications in health monitoring and patient rehabilitation. Recent research on HAR focuses on using smartphones due to their widespread use. However, this leads to inconvenient use, limited choice of sensors and inefficient use of resources, since smartphones are not designed for HAR. This paper presents the first HAR framework that can perform both online training and inference. The proposed framework starts with a novel technique that generates features using the fast Fourier and discrete wavelet transforms of a textile-based stretch sensor and accelerometer. Using these features, we design an artificial neural network classifier which is trained online using the policy gradient algorithm. Experiments on a low power IoT device (TI-CC2650 MCU) with nine users show 97.7% accuracy in identifying six activities and their transitions with less than 12.5 mW power consumption.

==> files/RL_update_old.tex <==
\noindent\textbf{Proposed Policy Gradient Update:}
In general, all the weights in the policy network 
can be updated after an epoch~\cite{sutton1998reinforcement2}.
This is useful when we start with an untrained network with random weights.
When a policy network is trained offline as in our example,
its first few layers generate broadly applicable intermediate features~\cite{liang2006fast}.
Consequently, we can update only the weights of the output layer
to take advantage of offline training and minimize the computation cost.
More precisely, we update the weights denoted by $\mathbf{\theta}$ in Figure~\ref{fig:rl_ann}
to tune our optimized ANN to individual users.

Since we use the value function as the objective,
the gradient of $J(\theta)$ is proportional to gradient of the policy~\cite{sutton1998reinforcement2}.
Using this result, the update equation for $\mathbf{\theta}$ is given as:
%
\begin{equation} \label{eq:weight_update}
 \mathbf{\theta}_{t+1} \doteq \mathbf{\theta}_t + \alpha r_t
\frac{\nabla_\mathbf{\theta} \pi(a_t|\hspace{0.5mm}\mathbf{h},\mathbf{\theta}_t)}{\pi(a_t|\hspace{0.5mm}\mathbf{h}, \mathbf{\theta}_t)}, 
\hspace{3mm} \alpha : \mathrm{Learning~rate}
\end{equation}
%
where $\mathbf{\theta}_{t}$ and $\mathbf{\theta}_{t+1}$ are
the current and updated weight matrices, respectively.
Similarly, $a_t$ is the current action at time $t$, $r_t$ is the corresponding reward, 
and $\mathbf{h}$ denotes the hidden layer outputs.
Hence, we need to compute the gradient of the policy to update the weights.  
Using Equation~\ref{Eq:policy}, we can express the partial derivative of the policy   
$\pi(a_t|\hspace{0.5mm}\mathbf{h}_t, \mathbf{\theta}_t)$ with respect to the weights $\theta_{j,i}$ as: 
%
\begin{equation}\label{eq:partial_derivative}
\frac{\partial \pi(a_t|\hspace{0.5mm}\mathbf{h}_t,\mathbf{\theta}_t)}{\partial\mathbf{\theta}_{j,i}} =
\frac{\partial \pi(a_t|\hspace{0.5mm}\mathbf{h}_t,\mathbf{\theta}_t)}{\partial 
O_{a_i}(\mathbf{h}_t,\mathbf{\theta})}
\frac{\partial 
O_{a_i}(\mathbf{h}_t,\mathbf{\theta})}{\partial\mathbf{\theta}_{j,i}}
\end{equation}
%
To facilitate partial update, we partition the weight into two disjoint sets
$\mathcal{S}_t$ and $\overline{\mathcal{S}_t}$.
$\mathcal{S}_t$ contains the weights with direct connections the output neuron for $a_t$,
while $\overline{\mathcal{S}_t}$ is the complementary set that contains the 
remaining weights in the output layer.
With this definition, we summarize the weight update rule in a theorem 
in order not to disrupt the flow of the paper with derivations.

\noindent \textbf{Weight Update Rule Theorem:} 
Given the current policy, reward and the learning rate $\alpha$, 
the weights in the output layer of the ANN given in Figure~\ref{fig:rl_ann} 
are updated online as follows:
%
\begin{equation}\label{eq:weight_update_final}
\theta_{t+1,j,i} \doteq
\begin{cases}
\mathbf{\theta}_{t,j,i} + \alpha r_t (1 - \pi(a_t|\hspace{0.5mm}\mathbf{h}_t,\theta_t)) \cdot 
h_{t,j}(\mathbf{X},\mathbf{\theta}_{in}) &
\mathbf{\theta}_{t,j,i} \in  \mathcal{S}_t\\
\mathbf{\theta}_{t,j,i} - \alpha r_t \pi(a_i|\hspace{0.5mm}\mathbf{h}_t,\theta_t)) \cdot 
h_{t,j}(\mathbf{X},\mathbf{\theta}_{in}) &
\mathbf{\theta}_{t,j,i} \in  \overline{\mathcal{S}_t}
\end{cases}
\end{equation}
%
\noindent \textbf{Proof:}  
When $\mathbf{\theta}_{t,j,i} \in  \mathcal{S}_t$, action $a_t$ corresponds to output $O_i(\mathbf{h},\mathbf{\theta})$.
Using the softmax function in Equation~\ref{Eq:policy}:
%
\begin{align}\label{eq:chain_rule1}
\frac{\partial \pi(a_t|\hspace{0.5mm}\mathbf{h}_t,\mathbf{\theta}_t)}{\partial 
O_{a_t}(\mathbf{h}_t,\mathbf{\theta}_t)} &=
\frac{e^{O_{a_t}(\mathbf{h}_t,\mathbf{\theta}_t)}}
	{\sum_{j=1}^{N_a}{e^{O_{a_j}(\mathbf{h}_t,\mathbf{\theta}_t)}} } -
\frac{\left( e^{O_{a_t}(\mathbf{h}_t,\mathbf{\theta}_t)}\right)^2}
	{\left( \sum_{j=1}^{N_a}{e^{O_{a_j}(\mathbf{h}_t,\mathbf{\theta}_t)}} 
	\right)^2 } 
	\nonumber \\
%
& = \pi(a_t|\hspace{0.5mm}\mathbf{h}_t,\mathbf{\theta}_t)\big(1 - \pi(a_t|\mathbf{h}_t,\mathbf{\theta}_t) \big)
\end{align}
%
Otherwise, i.e., $\mathbf{\theta}_{t,j,i} \notin  \mathcal{S}_t$,
we can express the partial derivative using Equation~\ref{Eq:policy} as:
%
\begin{align}\label{eq:chain_rule2}
\frac{\partial \pi(a_t|\mathbf{h}_t,\mathbf{\theta}_t)}{\partial 
O_i(\mathbf{h}_t,\mathbf{\theta}_t)} &=
- \frac{e^{O_{a_t}(\mathbf{h}_t,\mathbf{\theta}_t)} 
e^{O_{a_i}(\mathbf{h}_t,\mathbf{\theta}_t)}}
	{\left( \sum_{j=1}^{N_A}{e^{O_{a_j}(\mathbf{h}_t,\mathbf{\theta}_t)}} 
	\right)^2 
	} 
	%\nonumber \\
%& 
= -\pi(a_t|\mathbf{h}_t,\mathbf{\theta}_t) \pi(a_i|\mathbf{h}_t,\mathbf{\theta}_t)
\end{align}
%

The second term in Equation~\ref{eq:partial_derivative}, $\partial 
O_i(\mathbf{h}_t,\mathbf{\theta}_t)/ 
\partial\mathbf{\theta}_{j,i}$,
can be easily computed as $h_j(\mathbf{X},\mathbf{\theta}_{in})$ using 
Equation~\ref{eq:hidden_out}.
Hence, the weight update is the product of learning rate $\alpha$, reward $r_t$, 
$h_j(\mathbf{X},\mathbf{\theta}_{in})$ 
with Equation~\ref{eq:chain_rule1} if $\mathbf{\theta}_{t,j,i} \in  
\mathcal{S}_t$, 
with Equation~\ref{eq:chain_rule2} otherwise. 
%
Q.E.D~~$\square$

In summary, the weights of the output layer are updated onlnie using
Equation~\ref{eq:weight_update_final} after a user feedback. 
Detailed results for the improvement in accuracy
using RL are presented in Section~\ref{sec:rl_results}.

 

==> files/har_framework_old.tex <==
\section{\hspace{-4mm} Online Learning \lowercase{with} Policy Gradient} \label{sec:RL_approach} % Reinforcement Learning


%\subsection{Reinforcement Learning for New Users using Policy Gradients}
The trained ANN classifier is implemented on the IoT device
to recognize the human activities in real-time.
In addition to online inference, we propose a policy gradient based reinforcement learning (RL)
to continue training the classifier in the field.
Online training feature improves the recognition accuracy for new users
by as much as 32\% as demonstrated in our user studies.
%
%\textcolor{blue}{Once the offline training phase is complete, we deploy the ANN
%to the wearable device. At runtime, the user is asked to give feedback on the
%performance of the HAR. Using this feedback we continuously improve the weights
%of the ANN using reinforcement learning. Specifically, we use the policy
%gradient method, which updates the weights of the ANN in each iteration.}
We use the following definitions for the state, action, policy, and the reward.

\noindent\textbf{State:} Stretch sensor and accelerometer readings within a segment
are used as the continuous state space.
We process them as described in Section~\ref{sec:feature} to generate the input feature vector $\mathbf{X}$.

\noindent\textbf{Action:}
The ANN processes input features as shown in Figure~\ref{fig:rl_ann}
to generate the hidden layer outputs $\mathbf{h} = \{h_j, 1 \leq j \leq N_h+1\}$ 
and the activity probabilities $\pi(a_i|\mathbf{h}, \mathbf{\theta})$. 
Activity performed in each sensor data segment 
is interpreted as the action in our RL framework.

\noindent\textbf{Policy:}
The ANN learned during offline training outputs the policy
$\pi(a_i|\mathbf{h}, \mathbf{\theta}), 1 \leq i \leq N_A$ given in Equation~\ref{Eq:policy}.
It computes the probability of each action.

\noindent\textbf{Reward:}
Online training requires user feedback, which is defined as the reward function.
When no feedback is provided by the user, the weights of the network remain the same.
The user can give feedback upon completion of an activity such as walking,
which contains multiple segments (i.e., non-uniform action windows).
If the classification in this period is correct, a positive reward (in our implementation $+1$) is given.
Otherwise, the reward is negative ($-1$).
The sequence of segments for each reward is referred to as an \textit{epoch},
while the set of epochs in a given training session is called an \textit{episode}
following the RL terminology.

\noindent\textbf{Objective:}
The value function for a state is defined as the total reward
that can be earned starting from that state
by following the given policy until the end of the episode.
Our objective is to maximize the total reward $J(\mathbf{\theta})$
as a function of the classifier weights.

\noindent\textbf{Optimum Weight Update~\cite{sutton1998reinforcement2}:}
In order to find the change in the weights, we need to evaluate the gradient of the objective function.
When the value function is used as the objective,
the gradient of $J(\theta)$ is proportional to gradient of the policy
$\pi(a_i|\mathbf{X},
\mathbf{\theta})$~\cite{sutton1998reinforcement2}.
Using this result, the update equation for $\mathbf{\theta})$ is given as:
%
\begin{equation} \label{eq:weight_update}
\mathbf{\theta}_{t+1} \doteq \mathbf{\theta}_t + \alpha r_t
\frac{\nabla_\mathbf{\theta} \pi(a_t|\mathbf{X}_t,\mathbf{\theta}_t)}{\pi(a_t|\mathbf{X}_t, \mathbf{\theta}_t)}
\end{equation}
%
where $\mathbf{\theta}_{t}$ and $\mathbf{\theta}_{t+1}$ are
the current and updated weight matrices, respectively.
Similarly, $a_t$ is the current action, $\mathbf{X}_t$
is the current feature vector, and $r_t$ is the reward earned in the current time step.
Finally, $\alpha$ is the learning rate.


\noindent\textbf{Proposed Policy Gradient Update:}
In general, all the weights in the policy network can be updated using Equation~\ref{eq:weight_update}.
This is useful when we start with an untrained network.
When a policy network is trained offline,
its first few layers generate broadly applicable intermediate features~\cite{}.
Therefore, we update only the weights of the output layer
to tune our optimized ANN to individual users.
More precisely, we update only the weights denoted by $\mathbf{\theta}$ in~Figure~\ref{fig:rl_ann}
to take advantage of offline training and minimize the computation cost.

Suppose that user activity detected at time $t$ is denoted by $a_t$.
To facilitate partial update, we partition the weight into two disjoint sets
$\mathcal{S}_t$ and $\bar{\mathcal{S}_t}$.
$\mathcal{S}_t$ contains the weights with direct connections the output neuron for $a_t$,
while $\bar{\mathcal{S}_t}$ is the complementary set that contains the remaining weights.
With this definition, we can compute the the gradient of the policy
with respect to output layer weights $\theta_2$ as:
%
\begin{equation}\label{eq:rl_grad}
\frac{\partial \pi(a_t|\mathbf{X}_t,\mathbf{\theta}_t)}{\partial\mathbf{\theta}_{2,i}} =
\begin{cases}
\pi(a_t|\mathbf{X}_t,\mathbf{\theta}_t) (1 - \pi(a_t|\mathbf{X}_t,\mathbf{\theta}_t))
O_i(\mathbf{X},a_i,\mathbf{\theta}), &
\mathbf{\theta}_i \in \mathcal{S}_t \\
-\pi(a_t|\mathbf{X}_t,\mathbf{\theta}_t) \pi(a_j|\mathbf{X}_t,\mathbf{\theta}_t)
O_i(\mathbf{X},a_i,\mathbf{\theta}), &
\hspace{-7mm}
\theta_i \in
\bar{\mathcal{S}_t}, a_j\neq a_t
\end{cases}
\end{equation}
\textcolor{red}{where $O_i$ is the output of the hidden layer corresponding to
$\mathbf{\theta}_{2,i}$ and $a_j$ is action correspond to the output neuron connected to
$\mathbf{\theta}_{2,i}$}.
%
The proof of this result is given in the Appendix in order not to disrupt the flow.
%Using this result,
\textcolor{red}{We find the update equation for weights which are input to neuron corresponding to $a_t$ as (This is wrong, because we update all $\theta_2$ even if is it not in $S_1$)}:
%
\begin{equation}\label{eq:weight_update_final_old}
\theta_{t+1,i} \doteq
\begin{cases}
\theta_{t,i} + \alpha r_t (1 - \pi(A_t|x_t,\theta_t)) \cdot h_{o,i} &
\theta_i \in  \mathcal{S}_1\\
\theta_{t,i} - \alpha r_t \pi(a_j|x_t,\theta_t)) \cdot h_{o,i} &
\theta_i \in  \mathcal{S}_2\\
\theta_{t,i} & \text{otherwise}
\end{cases}
\end{equation}
%The proof of Equation~\ref{eq:rl_grad} is presented in the Appendix.

\begin{equation}\label{eq:weight_update_final}
\theta_{t+1,i} \doteq
\begin{cases}
\mathbf{\theta}_{t,i} + \alpha r_t (1 - \pi(a_t|\mathbf{X}_t,\theta_t)) \cdot O_i(\mathbf{X},a_i,\mathbf{\theta}) &
\mathbf{\theta}_i \in  \mathcal{S}_t\\
\mathbf{\theta}_{t,i} - \alpha r_t \pi(a_j|\mathbf{X},\theta_t)) \cdot O_i(\mathbf{X},a_i,\mathbf{\theta}) &
\mathbf{\theta}_i \in  \bar{\mathcal{S}_t}\\
\mathbf{\theta}_{t,i} & \text{otherwise}
\end{cases}
\end{equation}

At runtime, the weights of the output layer are updated using
Equation~\ref{eq:weight_update_final} after each window, based
on the feedback from the user. Detailed results for the improvement in accuracy
using RL are presented in Section~\ref{sec:rl_resuls} 

==> files/overview.tex <==
%\section{Preliminaries and Overview} \label{sec:overview}
%\subsection{Problem statement}
%\begin{itemize}
%	\item Identify states and transitions of human motion with greater than 
%	95\% 
%	accuracy without interfering with daily activities of a person
%	\item Adapt to individual user
%	\item Solution should not be limited to clinic. It should be a mobile and 
%	wearable that can operate with limited energy budget
%\end{itemize}
%
%\subsection{Challenges}
%One of the primary challenges 
%\begin{itemize}
%	\item The device should work for everybody and learn user behavior over time
%	\item Synchronization of multiple sensors and networking
%	\item Single sensor is not sufficient to get high accuracy. How to place 
%	multiple sensors on the body and how to combine data from them
%\end{itemize}

==> references/health_refs.tex <==
@article{arif2014better,
  title={Better physical activity classification using smartphone acceleration sensor},
  author={Arif, Muhammad and Bilal, Mohsin and Kattan, Ahmed and Ahamed, S Iqbal},
  journal={Journal of medical systems},
  volume={38},
  number={9},
  pages={95},
  year={2014}
}


@ONLINE{ODROID_Platforms,
	title={World Health Organization, Obesity and overweight. Fact Sheets},
	howpublished={Available [Online] \url{http://www.who.int/mediacentre/factsheets/fs311/en/.} Accessed 03/22/2018},
	year={2013}
}
